Constructing Large-Scale Real-World Benchmark Datasets for AIOps

Recently, AIOps (Artificial Intelligence for IT Operations) has been well studied in academia and industry to enable automated and effective software service management. Plenty of efforts have been dedicated to AIOps, including anomaly detection, root cause localization, incident management, etc. However, most existing works are evaluated on private datasets, so their generality and real performance cannot be guaranteed. The lack of public large-scale real-world datasets has prevented researchers and engineers from enhancing the development of AIOps. To tackle this dilemma, in this work, we introduce three public real-world, large-scale datasets about AIOps, mainly aiming at KPI anomaly detection, root cause localization on multi-dimensional data, and failure discovery and diagnosis. More importantly, we held three competitions in 2018/2019/2020 based on these datasets, attracting thousands of teams to participate. In the future, we will continue to publish more datasets and hold competitions to promote the development of AIOps further.

==> background.tex <==
\section{Background}
\nengwen{TODO}

==> makefile <==
MAIN_TEX = main.tex
TARGET_PDF = main.pdf
FIG_DIR = figs

TEX_FILES = $(shell find . -name '*.tex')
CROP_FIGURE_OPERATIONS = $(shell find '$(FIG_DIR)' -name '*.pdf' | sed -E 's/(.*)/\1.crop/g' | sed 's/ /\\ /g')

.SECONDARY:

.PHONY: crop phony_explicit build sync

build: $(TARGET_PDF);

crop: $(CROP_FIGURE_OPERATIONS);

clean:
	latexmk --output-directory=. -C

sync:
	(git add -u && git commit -m "$(date) local update") || echo nothing to commit
	git pull --no-edit
	git push


%.crop: % phony_explicit
	pdfcrop $< $<

.PHONY: build
${TARGET_PDF}: crop $(TEX_FILES)
	bash -c 'latexmk -C; latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX); latexmk -pdflatex -halt-on-error -interaction=nonstopmode $(MAIN_TEX)'

